Rethinking the Variational Interpretation of Nesterov's Accelerated Method

The continuous-time model of Nesterov's momentum provides a thought-provoking perspective for understanding the nature of the acceleration phenomenon in convex optimization. One of the main ideas in this line of research comes from the field of classical mechanics and proposes to link Nesterov's trajectory to the solution of a set of Euler-Lagrange equations relative to the so-called Bregman Lagrangian. In the last years, this approach led to the discovery of many new (stochastic) accelerated algorithms and provided a solid theoretical foundation for the design of structure-preserving accelerated methods. In this work, we revisit this idea and provide an in-depth analysis of the action relative to the Bregman Lagrangian from the point of view of calculus of variations. Our main finding is that, while Nesterov's method is a stationary point for the action, it is often not a minimizer but instead a saddle point for this functional in the space of differentiable curves. This finding challenges the main intuition behind the variational interpretation of Nesterov's method and provides additional insights into the intriguing geometry of accelerated paths.

==> gamma_conv.tex <==

Previous discussion focuses on the Lagrange functional defined on a \textit{finite} interval $[t_1, t_2]$. In this subsection we briefly explore the possibility of extending the variational problem into infinite time horizon.
\vspace{-2mm}
\paragraph{Importance of infinite time formulation}
Classical variational calculus assumes the functional to be defined on a finite interval $[t_1,t_2]$. Nevertheless, in continuous optimization, due to the existence of \textit{damping} in second order ODEs, the solution $Y$ is usually \textit{asymptotically} convergent to the optimal points $y^*$, i.e. $\underset{t \rightarrow \infty}{\lim} Y(t) = y^*$. We reckon therefore that there is a need to extend the finite-time variational formulation in Eq.~\ref{} into infinite-time horizon to cover this situation.
\vspace{-2mm}
\paragraph{$\Gamma$-convergence and variational convergence}
We tackle this by utilizing a sequential convergence argument for variational problems. Formally, suppose that there is a sequence of functionals $J_k$ defined on the space of $\mathcal{C}^1([t_1^{(k)},t_2^{(k)}],\bbR^d)$ functions and each one of $J_k$ admits a (global) minimum as
\begin{align}
    J^*_k = \min \{ J_k[Y]: Y \in \mathcal{C}^1([t_1^{(k)},t_2^{(k)}],\bbR^d) \},
\end{align}
we aim at studying the asymptotic behavior of the sequence $J_k$, i.e. when $k$ goes to infinity, the existence of a limit for $J_k$ as
\begin{align}
    J^*_\infty = \min \{ J_\infty(Y): Y \in \mathcal{C}^1([t_1^*,t_2^*],\bbR^d) \}.
\end{align}
where . The above problem can be tackled by employing the theory of $\Gamma$-convergence, which investigates the condition for the existence of such a limit $J_\infty[\cdot]$ and $J_\infty^*$. For a description of $\Gamma$-convergence theory, we provide a short introduction in Appendix. We also recommend \cite{braides2002gamma} for more details. Here we only informally state the following theorem regarding the existence for mininizer.
\begin{theorem}[Informal,\cite{braides2002gamma}] \label{thm:gamma-fundamental}
\end{theorem}
Now we apply the above theory to our analysis by constructing a sequence of $\{J_k\}$ as
\begin{align}
    \int_{t_1}^{t_2^{(k)}}L(Y,\dot{Y},t)dt
\end{align}
where $\underset{k\to\infty}{\lim}t_2^{(k)} = \infty$ and $L$ is the Bregman Lagrangian functional. Theorem~\ref{thm:gamma-fundamental} indicates that the limit of $\{J_k\}$ admits a minimizer/maximizer only if each $J_k$ admits a minimizer/maximizer. Nevertheless, as in the previous discussion, generally speaking, for Lagrangian $L(Y,\dot{Y},t)=t^3\left(\|\dot{Y}\|^2/2 - f(Y)\right)$ the above condition does not hold. Therefore we conclude that an infinite limit does not exist for Nesterov's path due to the ill-conditioned formulation of variational problem. 

